On the Design of Fast Convergent LDPC Codes: An Optimization Approach

The complexity-performance trade-off is a fundamental aspect of the design of low-density parity-check (LDPC) codes. In this paper, we consider LDPC codes for the binary erasure channel (BEC), use code rate for performance metric, and number of decoding iterations to achieve a certain residual erasure probability for complexity metric. We first propose a quite accurate approximation of the number of iterations for the BEC. Moreover, a simple but efficient utility function corresponding to the number of iterations is developed. Using the aforementioned approximation and the utility function, two optimization problems w.r.t. complexity are formulated to find the code degree distributions. We show that both optimization problems are convex. In particular, the problem with the proposed approximation belongs to the class of semi-infinite problems which are computationally challenging to be solved. However, the problem with the proposed utility function falls into the class of semi-definite programming (SDP) and thus, the global solution can be found efficiently using available SDP solvers. Numerical results reveal the superiority of the proposed code design compared to existing code designs from literature.

==> Fig/Approximation/Approximation.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{015}[cl][cl]{\matlabtextA Approximation in (11)\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA Exact number of iterations\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextB $R_2=0.48$}%
\psfrag{018}[cl][cl]{\matlabtextB $R_1=0.5$}%
\psfrag{019}[bc][bc]{\matlabtextB Number of Iterations, $N$}%
\psfrag{020}[tc][tc]{\matlabtextB Residual Erasure Probability, $P_N$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-6}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-5}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{-4}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{-3}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{005}[ct][ct]{\matlabtextC $10^{-1}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $20$}%
\psfrag{007}[rc][rc]{\matlabtextC $40$}%
\psfrag{008}[rc][rc]{\matlabtextC $60$}%
\psfrag{009}[rc][rc]{\matlabtextC $80$}%
\psfrag{010}[rc][rc]{\matlabtextC $100$}%
\psfrag{011}[rc][rc]{\matlabtextC $120$}%
\psfrag{012}[rc][rc]{\matlabtextC $140$}%
\psfrag{013}[rc][rc]{\matlabtextC $160$}%
\psfrag{014}[rc][rc]{\matlabtextC $180$}%
%
%% </ytick>

==> Fig/ComPer/ComPer.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA $\lambda(x)$ for COC, $R=0.4$\hspace{0.5em}}%
\psfrag{013}[cl][cl]{\matlabtextA $\lambda(x)$ for COC, $R=0.45$\hspace{0.5em}}%
\psfrag{014}[cl][cl]{\matlabtextA $\lambda(x)$ for POC, $R=0.4714$\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA $\psi(x)=2[1-(1-x)^{\frac{1}{7}}]$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[bc][bc]{\matlabtextB Functions $\psi(x)$ and $\lambda(x)$}%
\psfrag{017}[tc][tc]{\matlabtextB $x$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-5}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-4}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{-3}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{005}[ct][ct]{\matlabtextC $10^{0}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $10^{-6}$}%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-5}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{009}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{-1}$}%
%
%% </ytick>

==> Fig/Comparison/Comparison.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA POC in [24]\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA POC in [21]\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA COC code in [12]\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA Proposed COC with utility function (21)\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA Proposed COC with approximation (11)\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextB Upper limit}%
\psfrag{025}[bc][bc]{\matlabtextB Number of Iterations}%
\psfrag{026}[tc][tc]{\matlabtextB Rate to Capacity Ratio}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0.86$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.88$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.92$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.94$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.96$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.98$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $50$}%
\psfrag{010}[rc][rc]{\matlabtextC $100$}%
\psfrag{011}[rc][rc]{\matlabtextC $150$}%
\psfrag{012}[rc][rc]{\matlabtextC $200$}%
\psfrag{013}[rc][rc]{\matlabtextC $250$}%
\psfrag{014}[rc][rc]{\matlabtextC $300$}%
\psfrag{015}[rc][rc]{\matlabtextC $350$}%
\psfrag{016}[rc][rc]{\matlabtextC $400$}%
\psfrag{017}[rc][rc]{\matlabtextC $450$}%
\psfrag{018}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Fig/DiffDv/DiffDv.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA $d_v=30$\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA $d_v=16$\hspace{0.5em}}%
\psfrag{021}[cl][cl]{\matlabtextA $d_v=14$\hspace{0.5em}}%
\psfrag{022}[cl][cl]{\matlabtextA $d_v=12$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextB Upper limits}%
\psfrag{024}[bc][bc]{\matlabtextB Number of Iterations}%
\psfrag{025}[tc][tc]{\matlabtextB Rate to Capacity Ratio}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0.86$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.88$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.92$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.94$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.96$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.98$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextC $0$}%
\psfrag{009}[rc][rc]{\matlabtextC $50$}%
\psfrag{010}[rc][rc]{\matlabtextC $100$}%
\psfrag{011}[rc][rc]{\matlabtextC $150$}%
\psfrag{012}[rc][rc]{\matlabtextC $200$}%
\psfrag{013}[rc][rc]{\matlabtextC $250$}%
\psfrag{014}[rc][rc]{\matlabtextC $300$}%
\psfrag{015}[rc][rc]{\matlabtextC $350$}%
\psfrag{016}[rc][rc]{\matlabtextC $400$}%
\psfrag{017}[rc][rc]{\matlabtextC $450$}%
\psfrag{018}[rc][rc]{\matlabtextC $500$}%
%
%% </ytick>

==> Fig/ErrorCom/ErrorCom.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{014}[cl][cl]{\matlabtextA $\eta=10^{-5}$\hspace{0.5em}}%
\psfrag{015}[cl][cl]{\matlabtextA $\eta=10^{-3}$\hspace{0.5em}}%
\psfrag{016}[cl][cl]{\matlabtextA $\eta=10^{-2}$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextB $R_d=0.488$}%
\psfrag{018}[cl][cl]{\matlabtextB $R_d=0.485$}%
\psfrag{019}[bc][bc]{\matlabtextB Number of Iterations, $N$}%
\psfrag{020}[tc][tc]{\matlabtextB Residual Erasure Probability, $P_N$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $10^{-5}$}%
\psfrag{001}[ct][ct]{\matlabtextC $10^{-4}$}%
\psfrag{002}[ct][ct]{\matlabtextC $10^{-3}$}%
\psfrag{003}[ct][ct]{\matlabtextC $10^{-2}$}%
\psfrag{004}[ct][ct]{\matlabtextC $10^{-1}$}%
\psfrag{005}[ct][ct]{\matlabtextC $10^{0}$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextC $50$}%
\psfrag{007}[rc][rc]{\matlabtextC $100$}%
\psfrag{008}[rc][rc]{\matlabtextC $150$}%
\psfrag{009}[rc][rc]{\matlabtextC $200$}%
\psfrag{010}[rc][rc]{\matlabtextC $250$}%
\psfrag{011}[rc][rc]{\matlabtextC $300$}%
\psfrag{012}[rc][rc]{\matlabtextC $350$}%
\psfrag{013}[rc][rc]{\matlabtextC $400$}%
%
%% </ytick>

==> Fig/RateDv/RateDv.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA $\varepsilon=0.52$\hspace{0.5em}}%
\psfrag{019}[cl][cl]{\matlabtextA $\varepsilon=0.50$\hspace{0.5em}}%
\psfrag{020}[cl][cl]{\matlabtextA $\varepsilon=0.48$\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB Rate to Capacity Ratio}%
\psfrag{022}[tc][tc]{\matlabtextB Maximum Variable Degree, $d_v$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $5$}%
\psfrag{002}[ct][ct]{\matlabtextC $10$}%
\psfrag{003}[ct][ct]{\matlabtextC $15$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $25$}%
\psfrag{006}[ct][ct]{\matlabtextC $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $0$}%
\psfrag{008}[rc][rc]{\matlabtextC $0.1$}%
\psfrag{009}[rc][rc]{\matlabtextC $0.2$}%
\psfrag{010}[rc][rc]{\matlabtextC $0.3$}%
\psfrag{011}[rc][rc]{\matlabtextC $0.4$}%
\psfrag{012}[rc][rc]{\matlabtextC $0.5$}%
\psfrag{013}[rc][rc]{\matlabtextC $0.6$}%
\psfrag{014}[rc][rc]{\matlabtextC $0.7$}%
\psfrag{015}[rc][rc]{\matlabtextC $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextC $0.9$}%
\psfrag{017}[rc][rc]{\matlabtextC $1$}%
%
%% </ytick>
